openFEAT: Improving Speaker Identification by Open-set Few-shot Embedding Adaptation with Transformer

Household speaker identification with few enrollment utterances is an important yet challenging problem, especially when household members share similar voice characteristics and room acoustics. A common embedding space learned from a large number of speakers is not universally applicable for the optimal identification of every speaker in a household. In this work, we first formulate household speaker identification as a few-shot open-set recognition task and then propose a novel embedding adaptation framework to adapt speaker representations from the given universal embedding space to a household-specific embedding space using a set-to-set function, yielding better household speaker identification performance. With our algorithm, Open-set Few-shot Embedding Adaptation with Transformer (openFEAT), we observe that the speaker identification equal error rate (IEER) on simulated households with 2 to 7 hard-to-discriminate speakers is reduced by 23% to 31% relative.

==> main_table2.tex <==
\begin{table}[hbt]
\caption{The effect of constrastive learning loss weight ($\alpha$) on embedding adaptation model in hard households. $\beta$ is 0 in this study.}
\label{tab:ablation_alpha}
\resizebox{\linewidth}{!}{%
\begin{tabular}{c|rrrrr}
\toprule
  \multicolumn{1}{l|}{}  & \multicolumn{5}{c}{$\alpha$}   \\
  \multicolumn{1}{l|}{\textbf{n}} & \multicolumn{1}{c}{\textbf{0}} & \multicolumn{1}{c}{\textbf{0.1}} & \multicolumn{1}{c}{\textbf{0.5}} & \multicolumn{1}{c}{\textbf{1}} & \multicolumn{1}{c}{\textbf{5}} \\
\midrule
2 & 5.31$\pm$0.14& 5.43$\pm$0.12& \textbf{4.91$\pm$0.10} & 4.93$\pm$0.11& 5.71$\pm$0.13\\
3 & 7.12$\pm$0.12& 7.32$\pm$0.15& \textbf{6.75$\pm$0.08}& 6.89$\pm$0.12& 7.64$\pm$0.10 \\
4 & 9.04$\pm$0.12& 9.15$\pm$0.06& \textbf{8.56$\pm$0.08}& 8.69$\pm$0.11& 9.64$\pm$0.10 \\
5 & 10.58$\pm$0.14& 10.62$\pm$0.16  &\textbf{ 10.01$\pm$0.15} & 10.25$\pm$0.14& 11.23$\pm$0.14\\
6 & 11.88$\pm$0.14& 11.91$\pm$0.14 & \textbf{11.37$\pm$0.15} & 11.5$\pm$0.09& 12.67$\pm$0.12\\
7 & 13.09$\pm$0.28& 12.97$\pm$0.21 & \textbf{12.45$\pm$0.25} & 12.55$\pm$0.19& 13.76$\pm$0.22\\
\bottomrule
\end{tabular}}
\end{table}


==> main_table3.tex <==
\begin{table}[hbt]
\caption{The effect of open-set loss on embedding adaptation model ($\beta$) in hard households. $\alpha$ is 0.5 in this study.}
\label{tab:ablation_beta}
\resizebox{\linewidth}{!}{%
\begin{tabular}{c|rrrrr}
\toprule
    \multicolumn{1}{l|}{}  & \multicolumn{5}{c}{$\beta$} \\
    \multicolumn{1}{l|}{\textbf{n}} & \multicolumn{1}{c}{\textbf{0}} & \multicolumn{1}{c}{\textbf{0.01}} & \multicolumn{1}{c}{\textbf{0.1}} & \multicolumn{1}{c}{\textbf{0.5}} & \multicolumn{1}{c}{\textbf{1}} \\
\midrule
2& 4.91$\pm$0.10& 4.90$\pm$0.11& \textbf{4.49$\pm$0.13}& 4.94$\pm$0.09& 5.23$\pm$0.11  \\
3& 6.75$\pm$0.08& 6.81$\pm$0.12&\textbf{ 6.06$\pm$0.12}& 6.51$\pm$0.07& 6.95$\pm$0.14  \\
4& 8.56$\pm$0.08& 8.60$\pm$0.08& \textbf{7.67$\pm$0.14}& 8.15$\pm$0.11& 8.73$\pm$0.07  \\
5& 10.01$\pm$0.15& 10.06$\pm$0.14& \textbf{9.02$\pm$0.16}& 9.44$\pm$0.18& 10.05$\pm$0.15 \\
6& 11.37$\pm$0.15& 11.27$\pm$0.15& \textbf{10.30$\pm$0.15}& 10.62$\pm$0.15   & 11.24$\pm$0.14 \\
7& 12.45$\pm$0.25& 12.30$\pm$0.19 & \textbf{11.35$\pm$0.24}& 11.59$\pm$0.18   & 12.24$\pm$0.18 \\ 
\bottomrule
\end{tabular}}
\end{table}
